Topological susceptibility and the sampling of field space in $N_f=2$ lattice QCD simulations

We present a measurement of the topological susceptibility in two flavor QCD. In this observable, large autocorrelations are present and also sizable cutoff effects have to be faced in the continuum extrapolation. Within the statistical accuracy of the computation, the result agrees with the expectation from leading order chiral perturbation theory.

==> log.tex <==
\section{log-file}
\subsection{Rainer, 19.6. evening}
Some rephrasings in 3.2.2: read again.
\\
reference to that section in abstract and conclusions
\\[1ex]
{\bf the numbers in 3.2.2 need to be checked by somebody}

\subsection{Rainer's changes June 18}
sfb-number \\[2ex]
checked all of Stefan's changes. good. \\[2ex]
after (1.2) "...are now available" [irrelevant] \\[2ex]
p2 second paragraph: a few times "has been" -> "was" \\[2ex]
Discussion of tmQCD cont limit in footnote:
In this work, 
there is a single lattice spacing for the 2-flavor results. For $N_\mathrm{f}=$2+1+1
three lattice spacings are present but the continuum extrapolation assumes 
the susceptibility to vanish in the chiral limit at fixed lattice spacing, see our 
discussion in \sect{s:cont}.
\\[2ex]
added t0, t1 after (2.4)
\\[2ex]
caption table 1: ...the total statistics in molecular dynamics units (MDU) ...
\begin{equation}
\tauint = \frac{1}{2} + \sum_{\tau=1}^{W-1} \rho(\tau) + \tauexp \rho(W) \ .
\end{equation}
For this method an estimate of the largest time constant $\tauexp$ in the 
simulation is needed....
\\[2ex]
removed "good" in:\\
 \Fig{fig:autocorr-1} shows the dependence of the
autocorrelation functions on the lattice spacing. While the rescaling of the
Monte Carlo time with $t_0$ confirms the scaling properties ...
\\[2ex]
after (3.5):\\
The correlator $\langle \bar q(z_0) \bar q(x_0+z_0) \rangle$ will be studied below.
As we will see, it falls off quickly for large $x_0$ such
that the sum can be truncated at moderate $r$. 
\\[2ex]
expectation value in:
\\
influence of the boundaries in $\langle \bar q(x_0)^2 \rangle $
is visible with the present accuray up to 1.5~fm.
\\[2ex]
below: 
No differences {\bf to B6 } ...
\\[2ex]
end sect. 3.3.:\\
which we attribute to our limited sampling of the tails.
\\[2ex]
after (3.6):\\
...With the lattice spacing {\bf determined from}
the kaon decay constant...
\\[2ex]
end of first para of 4. :\\
... whereas the other slow modes, as seen, e.g., in  $E(t_0)$, do not
profit.
\\[2ex]
long acknowledgements

\subsection{Stefan's changes June 17}
Changed affiliation. {\bf Rainer check}\\[2ex]
before eq 2.2: topological density -> topological charge density\\[2ex]
before eq 2.3: energy -> energy density\\[2ex]
Inserted footnote citing the CLS webpage\\[2ex]
section 2.2: replaced behaviour -> behavior\\[2ex]
last paragr of sec2 : as it will be -> as will be\\[2ex]
Section 3.1: I agree with the text, small rephraseing after "Thridly"\\
as a consequence removed "Old text" footnote
\\[2ex]
after eq 3.3 : removed the stray r=T/2\\[2ex]
before eq 3.8: {\bf rephrased discussion of WChPT}\\[2ex]
footnote : indepted to xxx to -> indepted to xxx for\\[3ex]
{\color{red} Footnote comparing the DelDebbio to other results}
\\[2ex]
caption table 1: ...the total statistics in molecular dynamics units (MDU) ...
\begin{equation}
\tauint = \frac{1}{2} + \sum_{\tau=1}^{W-1} \rho(\tau) + \tauexp \rho(W) \ .
\end{equation}
For this method an estimate of the largest time constant $\tauexp$ in the 
simulation is needed....
\\[2ex]

\subsection{MB, 17.6}
DESY preprint. Some words adjusted to American (e.g. flavour into flavor).
I've changed symbols in plots such that they are consistent (e.g. triangle
for all point with coarsest spacing). I've filled table 3 with the oB6 value.


\subsection{RS, 11.6.}
A number of changes in sect. 3 . Did not keep track of
details. 

\subsection{RS, 26.5.}
wordings second to last para p1, and in the two 
last paras of p2.
\\[2ex]
Removed "then" in beginning of para 3 sect2
\\[2ex]
Caption table 1
\\[2ex]
sect. 2.2: \\
For this method an estimate of the largest time constant in the simulation is needed.
Since the dynamics of  parity even and parity odd observables 
decouples\cite{Schaefer:2010hu},
we can restrict ourselves to even ones. Then $Q^2(t)$ is an obvious
candidate to look for the largest time constant, but we also investigate $E(t)$.
\\[2ex]
Caption fig. 2 .
\\[2ex]
The results of the integrated
autocorrelation times (summed up to $R\tau \approx 40 t_0$) for $Q^2$ and $E$ are given in \tab{tab:tauint}.
\\
{\bf is that true?}
\\[2ex]
\begin{equation}
\tauint = \frac{1}{2} \sum_{\tau=0}^{W-1} \rho(\tau) + \tauexp \rho(W) \ .
\end{equation}
above eq.(2.9):
\\
Since $E$ has the largest autocorrelations in our range of lattice spacings
and its autocorrelation function is approximately an exponential function,
we can identify  $\tauint(E)$ with $\tauexp$ at the current level of accuracy.
\\[2ex]
sect.3 \\
some small changes 
\\ to complete:
($\sqrt{t_0} m_\pi \sim \ldots$)
\\[2ex]
above 3.2.1:
\\
The reason is that the statistics is roughly the 
same. Furthermore, the reweighting factors of the twisted mass 
reweighting employed in the oB6 ensemble decouple almost completely
from pure gluonic observable, like the charge.
\\
or: ``... contribute very little to the errors of  
pure gluonic observable, like the charge ...''
\\[2ex]
sects 3.3-3.4 a few little things
\\[2ex]
{\color{red} 
Rainer had a complaint from
Wuppertal about their precise quenched suscept. {\bf Stefan put in a footnote, please check!}}
\\[3ex]


{\bf Conclusion}\\
Rephrased second paragraph concernign WChPT and continuum limit.


